Lateral Gene Transfer, Rearrangement and Reconciliation

Background. Models of ancestral gene order reconstruction have progressively integrated different evolutionary patterns and processes such as unequal gene content, gene duplications, and implicitly sequence evolution via reconciled gene trees. In unicellular organisms, these models have so far ignored lateral gene transfer, even though it can have an important confounding effect on such models, as well as a rich source of information on the function of genes through the detection of transfers of entire clusters of genes. Result. We report an algorithm together with its implementation, DeCoLT, that reconstructs ancestral genome organization based on reconciled gene trees which summarize information on sequence evolution, gene origination, duplication, loss, and lateral transfer. DeCoLT finds in polynomial time the minimum number of rearrangements, computed as the number of gains and breakages of adjacencies between pairs of genes. We apply DeCoLT to 1099 gene families from 36 cyanobacteria genomes. Conclusion. DeCoLT is able to reconstruct adjacencies in 35 ancestral bacterial genomes with a thousand genes families in a few hours, and detects clusters of co-transferred genes. As there is no constraint on genome organization, adjacencies can be generalized to any relationship between genes to reconstruct ancestral interactions, functions or complexes with the same framework.

==> Makefile <==
PDFLATEX = pdflatex
LATEX = latex
RM = rm -f

default:
	make figs
	make rcg_2013

%:
	$(PDFLATEX) $(@).tex
	bibtex $(@)
	$(PDFLATEX) $(@).tex
	$(PDFLATEX) $(@).tex
	make clean

figs:
	if test -s figures/fig-1.pdf; then echo "figures already built"; else cd figures; make; fi;

clean:
	$(RM) *~ *\# *.aux *.log *.bbl *.blg *.dvi *.ps

scour:
	make clean
	$(RM) *.pdf
	cd figures; make scour

#################################################################

### latex diff stuff

OLD=oldversion
NEW=rcg_2013
diff:
	latexdiff-so -V $(OLD).tex $(NEW).tex > thediff.tex
	make thediff

### latex template

latextemplate:
	$(LATEX) $(@).tex
	bibtex $(@)
	$(LATEX) $(@).tex
	$(LATEX) $(@).tex
	dvips -t letter $(@).dvi -o $(@).ps
	ps2pdf $(@).ps $(@).pdf
	make clean

